Fairness for All: Investigating Harms to Within-Group Individuals in Producer Fairness Re-ranking Optimization -- A Reproducibility Study

Recommender systems are widely used to provide personalized recommendations to users. Recent research has shown that recommender systems may be subject to different types of biases, such as popularity bias, leading to an uneven distribution of recommendation exposure among producer groups. To mitigate this, producer-centered fairness re-ranking (PFR) approaches have been proposed to ensure equitable recommendation utility across groups. However, these approaches overlook the harm they may cause to within-group individuals associated with colder items, which are items with few or no interactions. This study reproduces previous PFR approaches and shows that they significantly harm colder items, leading to a fairness gap for these items in both advantaged and disadvantaged groups. Surprisingly, the unfair base recommendation models were providing greater exposure opportunities to these individual cold items, even though at the group level, they appeared to be unfair. To address this issue, the study proposes an amendment to the PFR approach that regulates the number of colder items recommended by the system. This modification achieves a balance between accuracy and producer fairness while optimizing the selection of colder items within each group, thereby preventing or reducing harm to within-group individuals and augmenting the novelty of all recommended items. The proposed method is able to register an increase in sub-group fairness (SGF) from 0.3104 to 0.3782, 0.6156, and 0.9442 while also improving group-level fairness (GF) (112% and 37% with respect to base models and traditional PFR). Moreover, the proposed method achieves these improvements with minimal or no reduction in accuracy (or even an increase sometimes). We evaluate the proposed method on various recommendation datasets and demonstrate promising results independent of the underlying model or datasets.

==> sections/4-prob-solution.tex <==



\section{Problem formulation and proposed solution}




%\subsection{Related Work}
%Producer fairness is at the center of several RS research efforts \cite{geyik2019fairness}. \citet{gomez2021winner} analyze educational RS, observe an overexposure of courses from the most represented countries in the data— thus generating unfairness for teachers outside that country— and propose an approach that regulates visibility and exposure. \citet{kirnap2021estimation} consider three fairness representation targets used in literature: (1) exposure parity, (2) proportionality to the corpus presence, (3)  proportionality to the relevance, besides reporting and estimating the following four divergence-based fairness metrics: (1) difference, (2) absolute difference, (3) squared difference, (4) KL divergence. Another approach by \citet{wu2021tfrom} consists of building two post-processing heuristic algorithms—offline and online—based on a knapsack optimization model with fairness as the objective.

%For producers, users' needs are one of the pillars to be fulfilled: calibration is an important fairness-derived concept that aims to maximize a user's accuracy while keeping the preferred recommendation ratio, i.e. if the user watches 70 romance movies and 30 action movies, then it is reasonable to expect the personalized list of recommended movies to be comprised of about 70\% romance and 30\% action movies as well \cite{steck2018calibrated}. \citet{naghiaei2022towards} propose a confidence-aware optimization-based re-ranking algorithm to find the balance between calibration, relevance, and item diversity, while simultaneously accounting for calibration confidence based on user profile size.


\subsection{Problem Formulation}
%Let $\mathcal{U}$ and $\mathcal{I}$ be the set of users and items with size $n$ and $m$, respectively. Typically, a recommender system provides a user, $u \in \mathcal{U}$, a list of top-N items, $L_N(u)$ according to a set of relevance scores, $s \in S^{n\times N}$. Further, we have a binary set of category information which describes a certain property of the items, $c \in C^{n\times N}$. The objective is to generate a new fair list, $L^{F}_K(u)$ from the original unfair top-N recommended items $L_N(u)$, with $L^{F}_K(u) \subset L_N(u) \ \ where \ \ K \leq N$ such that the new list has the best balance between item relevance, fairness and novelty for the specific user.

Let $\mathcal{U}$ and $\mathcal{I}$ represent the set of $n$ users and $m$ items, respectively. A recommender system typically offers a user, $u \in \mathcal{U}$, with a list of the top-$N$ items, $L_N(u)$, based on a set of relevance scores, $s \in S^{n\times N}$. %\yashar{Not sure we need it} 
%In addition, a binary set of category information,  $c \in C^{n\times N}$, that describes a given attribute of the objects.\yashar{till here}
The goal is to learn a new fair list, $L^{F}_K(u)$, from the original unfair top-$N$ suggested items, $L^{F}_K(u) \subset L_N(u) \ \ where \ \ K \leq N$  such that the new list has the optimal balance of item relevance, fairness, and novelty for the particular user.

In $L_N(u)$, item $I_1$ has a higher ranking with respect to item $I_2$ based only on its score $s_{u1} > s_{u2}$. This does not take into account other crucial marketplace objectives, such as the one considered in this work. In this work, we define a binary decision vector $\mathbf{x}_{i}(u)$ for each user $u \in \mathcal{U}$, that has a value of 1 when the item ranked $i$ in $L_N(u)$ has also ranked in the fair-novel list $L_K(u)$, and 0 otherwise. $L_K(u)$ for user $u$ can be represented as $[\mathbf{x}_{1},\mathbf{x}_{2},...,\mathbf{x}_{N}]$ when $\sum_{i=1}^{N}{\mathbf{x}_{i}} = K $, $K\leq N$. Below we define our mixed-integer linear programming re-ranking algorithm which optimizes the values of $\mathbf{x}_{i}(u)$ chosen for ranking in $L_K(u)$.

%In the following, we assume $\mathcal{G}$ be the set of group labels and $\mathcal{I}_g \subset \mathcal{I}$ be the subset of items with group label $g \in \mathcal{G}$. We analyze the case when two groups split the corpus (i.e., $\mathcal{G} = \{A, B\}$).

%Given a ranking $L_N(u)$, a group-based fair ranking metric is composedof three computations: (a) measuring the group representation in
%��, (b) defining a target group representation for that query, and(c) comparing the group representation in �� with the target grouprepresentation

%, and D, D is a partition of D).e consider the situation where there are two groups thatpartition the corpus (i.e. G = {��, ��} and {D��, D��} is a partition oD).
%We define a binary decision matrix $A=[A_{ui}]_{n \times N}$ with value 1 when the item ranked $i$ in $L_N(u)$ is recommended to user $u$ in the new fairness-aware recommendation list, i.e., $L^F_K(u)$ and 0 otherwise. Hence, the fair top-K recommendation list to user $u$, can be represented as $[A_{u1},A_{u2},...,A_{uN}]$ when $\sum_{i=1}^{N}{A_{ui}} = K $, $K\leq N$.
%We discuss below an  optimization framework to calculate optimal values for matrix $A$ and re-rank the original unfair recommendation list.



\subsection{Fair Exposure of Items and Producers}

We assume $\mathcal{G}$ be the set of group labels and $\mathcal{I}_g \subset \mathcal{I}$ be the subset of items with group label $g \in \mathcal{G}$. We analyze the case when two groups split the corpus (i.e., $\mathcal{G} = \{A, B\}$ and $\{I_A, I_B\}$ is a partition of
$\mathcal{I}$). This paper focuses on the scenario when item groups are short-head vs. long-tail items. However, the methodology is universal and may be applied to any protected group class.

Given a top-$N$ recommendation list offered to user $u$, i.e., $L_N({u})$, a group-based fair recommendation should be computed at the \textit{user level} based on three main components:  (a) measuring the group representation offered by the recommendation model $p_m$, (b) defining a target group representation for that user $p_t$, and
(c) comparing the group representation with the target group representation

\begin{equation}
\begin{aligned}
% \begin{small}
PF_c (X, I_A, I_B) = \Gamma (p_m, p_t)
% \end{small}
\end{aligned}
\end{equation}

\yashar{@vittorio/giovanni: Please look at the variable $(X, I_A, I_B)$, I did not check carefully what is the role of $X$, but make sense somehow. Moreover, we may be able to use $(X, A, B)$ as well.}



where $PF$ is a metric that quantifies item groups’ exposition in the recommendation list decision $X$ and is computed at the user level. Here, $p_m$ measures the exposition of items and producer, and can be computed based on two types of benefits, exposure, and relevance, both of which can be binary or graded \cite{gomez2022provider}. Given that suppliers' primary objective is their products' visibility, this study focuses its attention exclusively on the (binary) exposure dimension, leaving the other producer fairness constraints for future work. To measure $p_t$, while Kirnap suggests diverse approaches for gauging fairness, the vast majority of prior work on fairness optimization, for instance, xx, xxx, use the simplest uniform target representation (equal exposition). Extending this definition in this work, motivated by xxx,  we present a framework that permits the optimization of a flexible notion of fairness, as determined by the producer to be of interest.

\begin{enumerate}
    \item \textbf{Uniform.} which is equal to the uniform probability distribution (in Table 2 we denote it with $PF_{eq}$);
    \item \textbf{Proportional.} using the basic principle that the degree of item exposition should be proportional to the number of items in the corpus that belong to a particular group, supporting the concept of reasonable disparity in producer item exposition. When item exposition is calibrated based on item exposition, we refer to this concept as producer-size calibrated (in Table xxx we denote it with $PF_{prop}$); 
\end{enumerate}
Similarly, the $\Gamma$ function is based on the notions expressed by \cite{kirnap2021estimation}'s equations (4) and (6) and it can use several different metrics. In this work, we adopted \cite{kirnap2021estimation}'s equation (4) as well:

 \begin{equation}
\Delta_{abs} = \sum_{\textit{g}\in\mathcal{G}}\left | \textbf{P}_{g} - \tilde{\textbf{P}}_{g} \right |
 \end{equation}
 

\subsection{Enhancing Exposition of Novel and Niche Items}

 One technique to achieve novelty is to provide personalized recommendations that include novel or niche products, thereby promoting the less popular (also referred to as \textit{cold-start}) items in the inventory.

 \begin{equation}
N(i | i\in\mathcal{C}) = \sum_{i\in\mathcal{C}}-log_2(P_i)
 \end{equation}

We compute a novelty score $N_{i}$ at the item level by referring to the popularity score $P_{i}$ of the single item, based on its occurrence throughout the dataset's interactions.




\subsection{Proposed Solution}



In this section, we will use the top-N recommendation list and relevance scores provided by the traditional unfair recommendation algorithm as a baseline. We apply a re-ranking post-hoc algorithm to maximize the total sum of relevance scores while minimizing the deviation from fairness on the producer, $\mathbf{DCF}$. We can formulate the fairness-aware optimization problem given the binary decision matrix, A, as:

\begin{small}
\begin{equation}
\begin{aligned}
% \begin{small}
\max_{X_{i}} \quad & \sum_{i=1}^{N}{S_{i}.N_{i}^{\gamma}.X_{i}} - \lambda. PF_{c}(X,\mathcal{I})\\
\textrm{s.t.} \quad & \sum_{i=1}^{N}{X_{i}} = K, X_{i} \in{\{0,1\}}\\
% \end{small}
\end{aligned}
\label{eq:optimization}
\end{equation}
\end{small}

The solution to above optimization problem would recommend exactly $K$ items to each user while maximizing the summation of preference scores and penalizing deviation from fairness. $ 0 \leq \lambda \leq 1$ is the hyper parameters that would be selected based on the application and would assign how much weight is given to each fairness deviation concern. Note that if the value of $\lambda$ is equal to $0$ then the optimal solution will be the same as the baseline recommendation system list, that is, $L^{F}_K(u) = L_K(u)$. The effect of different values for $\lambda$ and $\gamma$ are studied in the ablation study section. Parity between groups is defined as the ideal representation of the fairness in the model but is not enforced as a constraint in our optimization to avoid resulting in diminishing the total model accuracy in a significant way.

The optimization problem above is a mixed-integer linear programming (MILP) and a known NP-hard problem. Although MILP cannot be generally solved optimally in polynomial time, there exists many fast heuristic algorithms and industrial optimization solvers that would provide a good feasible solution in practice\footnote{eg Gurobi solver at \url{https://www.gurobi.com}}. The MILP proposed optimization at Equation~\ref{eq:optimization} can be reduced to a special case of Knapsack problem where the goal is to select items for each user that would maximize the total score in which each item has a weight equal to 1 and the total weight is constrained by fixed size K. Since each item has the same weight in this instance of Knapsack problem, we can solve it optimally by a greedy algorithm in polynomial time. Now we are ready to propose the Fair Re-ranking Greedy algorithm (Algorithm~\ref{alg:LBP}) that would give the optimal solution for the optimization problem in Equation~\ref{eq:optimization}. Alternatively, we can relax the binary constraint of variables to fractional variables with boundary constraints \ie $0\leq A_{ui}\leq1$ and solve the relaxed optimization problem in polynomial time. The algorithm based on optimization is presented in Algorithm~\ref{alg:optmization}.

\begin{algorithm}
	\DontPrintSemicolon
	\SetAlgoLined
	\SetKwInOut{Input}{\textit{$\mathcal{U},\mathcal{I}, \lambda_1,\lambda_2, K$}}\SetKwInOut{Output}{Output}
	\Input{\textit{$\mathcal{U},\mathcal{I}, \lambda_1,\lambda_2, K$}}
	\Output{Item recommendation matrix  {${A}^*$}}
	\tcc{${A}^*$ is a $n\times N$  binary matrix with elements $1$ when the item is recommended to the user and $0$ otherwise .}
	S $\leftarrow$ Run baseline algorithm and store the relevance score matrix for top-N items for each user \;
	\tcc{$S$ is a $n\times N$  matrix representing the predicted relevance score generated by unfair baseline algorithms for each user-item pair}
	Formulate the Optimization Problem as an Integer Programming following equation \ref{eq:optimization} \;
	Solve Relaxed Linear Programming with added boundary constraint $0\leq A_{ui}\leq1$, $\forall u\in \mathcal{U} , \forall i \in \{1,2,...,N \}$ \;
	\Return{$A^*$}
	\caption{The Fair Re-ranking Optimization}
	\label{alg:optmization}
\end{algorithm}

\begin{algorithm}
	\DontPrintSemicolon
	\SetAlgoLined
	\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
	\Input{\textit{$\mathcal{U},\mathcal{I}, \lambda_1,\lambda_2, K$}}
	\Output{Fair top-K recommendation list  {$L^{F}_K$}}
	
	S $\leftarrow$ Run baseline algorithm and store the relevance score matrix for top-N items for each user  \;
	$UG_{u}$ $\leftarrow$ Binary vector with elements of $1$ when user $u \in \mathcal{U}$ is in the protected group and $-1$ otherwise \;
	$PG_{i}$ $\leftarrow$ Binary vector with elements of $1$ when item ranked $i$ in the traditional top-N recommendation list, ${L}_N(u)$, is in the protected group and $-1$ otherwise \;

	\tcc{Protected groups are the underrepresented groups in baseline algorithms such as unpopular items }
	    
	\ForEach{$u\in \mathcal{U}$}{
        \ForEach{$i\in \{1,2,...,N\}$} {
            $CF_{ui} \leftarrow UG_{u} \times \mathcal{MC}(u,i)$ \;
            $PF_{ui} \leftarrow PG_{i} \times \mathcal{MP}(u,i)$ \;
		    $\hat{S}_{ui}\leftarrow S_{ui} + \lambda_1 CF_{ui} + \lambda_2 PF_{ui} $
		    
		    }
		}
   $L^{F}_K(u)$ $\leftarrow$ Sort matrix $\hat{S}$ along the rows axis and select top-$K$ items for recommendation to each users, $\forall$ $u\in \mathcal{U}$ \;
	\Return{$L^{F}_K(u)$}
	\caption{The Fair Re-ranking Greedy Algorithm}
	\label{alg:LBP}
\end{algorithm}

We finally discuss the time complexity of the Fair Re-ranking Greedy algorithm.

\begin{lemma}
The time complexity of the proposed re-ranking algorithm has a worst case bound of $\mathcal{O}(n\times N)$
\end{lemma}

\begin{proof}
The first 3 lines of the algorithm will store the traditional relevance score matrix for Top-N items and store the protected groups in consumers and providers which can be done in linear time $\mathcal{O}(n + m)$. The second part in line 4-10 is to re-score all elements in the original relevance matrix by accounting for fairness measures which needs $\mathcal{O}(n \times N)$ operations in constant time. Lastly, we will sort the new relevance matrix for all users and select top-K items for recommendation. Using max-heap the worst case time complexity is $\mathcal{O}(N + K \log(K))$. Hence, considering $N$ and $K$ are much smaller than $n$, the total time complexity is $\mathcal{O}(n \times N)$ 
\end{proof}

==> sections/5-exp-results.tex <==
\section{Experiments and Results}

In this section, we first describe the experimental setup and datasets used, then we present the results we obtained throughout our experiments.

\subsection{Experimental Setup} 
 \textbf{Datasets.} To evaluate the generalizability of the proposed approach across other domains/datasets, we used five datasets: \datasetA, \datasetB, \datasetC, \datasetD, and \datasetD, all public and from popular domains such as Movies, E-commerce, Music and Business. The first three contain explicit ratings from 1-5, and after applying \textit{k}-core filtering (\textit{k = 10}) on Prime Pantry and Luxury Beauty they contain respectively 944, 6049, 2719 users and 1683, 4387, 1028 items. The last two, LastFM and Foursquare, are implicit and contain, respectively, 1867, 1083 users and 1529, 5135 items after \textit{k}-core filtering (\textit{k = 10}).

% The datasets we use are MovieLens100K, Amazon Prime Pantry, Amazon Luxury Beauty, LastFM, and Foursquare, all public and from popular domains such as Movies, E-commerce, Music and Business. The first three contain explicit ratings from 1-5, and after applying \textit{k}-core filtering (\textit{k = 10}) on Prime Pantry and Luxury Beauty they contain respectively 944, 6049, 2719 users and 1683, 4387, 1028 items. The last two, LastFM and Foursquare, are implicit and contain respectively 1867, 1083 users and 1529, 5135 items after \textit{k}-core filtering (\textit{k = 10}).

\vspace{0.5em}\noindent\textbf{Evaluation Method.} \giovanni{Stable} Our settings involve a train-validation-test split for the data with ratios 80\%, 10\%, and 10\%, respectively. For the purpose of re-ranking, we divide our items into two different groups based on their popularity, selecting the top 20\% in terms of interactions as the short-head or popular items and the bottom 80\% as the long-tail or unpopular items. Furthermore, we compute a novelty score for each item, characterizing it more as colder or warmer. 
\vspace{0.5em}

\vittorio{probably to be removed}\noindent\textbf{Sampled Datasets.} Simultaneously, we generate sampled recommendation datasets to further expand our analytical and experimental resources and test the performance of our system in the scenario of changing data characteristics. The sampled versions are generated starting from one of the main datasets we use, LastFM.

\vittorio{the previous one is the right one, this we can remove (I'm leaving it for the last part where you described mCPF, should we add something similar?)}\textbf{Evaluation Method.}
For the experiments, we randomly split each dataset into train, validation, and test sets in 70\%, 10\%, and 20\% respectively, and all the baseline models share these datasets for training and evaluation. For the re-ranking experiment, we categorize both users and items into two groups \cite{li2021user,abdollahpouri2019unfairness}. For users, we select the top 5\% users based on the number of interaction/level of activity from the training set as the active group and the rest as the inactive group. For items, we select top 20\% of items according to the number of interactions they received from the training set as the popular items, \ie short-head items, and the rest as the unpopular items or long-tail items. In addition, we define Consumer-Producer fairness evaluation (mCPF) metric to evaluate the overall performance of models \wrt two-sided fairness. mCPF computes the weighted average deviation of provider fairness (DPF) and deviation of consumer fairness (DCF), \ie $mCPF(w) = w \cdot DPF + (1-w) \cdot DCF$, where $w$ is a weighting parameter that can be selected by the system designer depending on the application or priority for each fairness aspect of the \textit{marketplace}. DCF and DPF are defined in Equations \ref{eq:dpf} and \ref{eq:dcf}, respectively, and the lowest value for mCPF shows the fairest model. To select the model parameters, $\lambda_1$ and $\lambda_2$, we treat them as a hyper parameter and set them to the value that maximize the average values of mCPF and overall nDCG for each dataset and model.

\vspace{0.5em}\noindent\textbf{Baselines.} \giovanni{Stable}
We compare the performance of our fairness method on several recommendation approaches, from traditional to deep recommendation models. The introduction of baselines are as the following:

\begin{itemize}
    \item \textbf{BPR} \cite{10.5555/1795114.1795167}: This method is generic optimization criterion for personalized ranking
    \item \textbf{MultiVAE} \cite{10.1145/3178876.3186150}: This method is a non-linear probabilistic model, which extends variational autoencoders (VAEs) to collaborative filtering for implicit feedback.
    \item \textbf{NeuMF} \cite{10.1145/3038912.3052569}: This algorithm learns user and item features using multi-layer perceptron (MLP) on one side and matrix factorization (MF) from another side, then applies non-linear activation functions to train the mapping between users and items features that are concatenated from MLP and MF layers.
    \item \textbf{NGCF} \cite{10.1145/3331184.3331267}: This method is a graph model which exploits the user-item graph structure by propagating embeddings on it.
    \item \textbf{LightGCN} \cite{10.1145/3397271.3401063}:
    This method is a Graph Convolution Network model,  learns user and item embeddings by linearly propagating them on the user-item interaction graph.
\end{itemize}

\vittorio{edit this}\noindent We compare our proposed fair CP re-ranking algorithm with unilateral fairness models, C and P-fairness re-ranking on top of the baselines to show how our method can achieve the desirable performance on fairness metrics in both stakeholders and overall recommendation performance (accuracy and beyond-accuracy).

\partitle{Evaluation Settings.} \giovanni{Added list of hyperparams}
We conducted hyperparameter tuning for both traditional and deep recommendation models, using a greedy search strategy. Best
models are selected based on the performance on the validation set. The hyperparameters for each model follow in detail:
\begin{itemize}
    \item \textbf{BPR}: embedding size and learning rate, with 20 different trials;
    \item \textbf{MultiVAE}:  learning rate,  latent dimension, mlp hidden size and drop-out propability, with 90 different trials;
    \item \textbf{NeuMF}: learning rate, drop-out probability, mlp hidden size, mf embedding size, and mlp embedding size, with 108 different trials;
    \item \textbf{NGCF}: embedding size, learning rate,  latent dimension, reg. weight, message dropout, with 108 different trials;
    \item \textbf{LightGCN}:
    embedding size, learning rate,  number of layers, and reg. weight, with 270 different trials;
\end{itemize}



\subsection{Results}


To gain a better understanding of the merits of the proposed CP fairness optimization framework, through the course of experiments, we intend to answer the following evaluation questions:
\begin{description}
    \item \textbf{Q1}: Comparing the baseline CF models to the proposed system, how does the proposed approach fulfill the requirement for PFairness using calibrated notion and equality, novelty, and overall system accuracy?
    \item \textbf{Q2}: How do the introduced fairness- and novelty-related parameters influence the interplay between the aforementioned metrics, and is there an ideal trade-off? Is it possible to improve the system's novelty and fairness by increasing these parameters without compromising other evaluation goals?
\end{description}

   % How does \underline{one-sided} fairness optimization (C-fairness~\cite{li2021user,islam2021debiasing} or P-Fairness~\cite{gomez2022provider,boratto2021interplay}), which has been the main subject of \underline{previous research}, affect the fairness constraints of other stakeholders, for example, if maximizing P-Fairness (i.e., reducing DPF) results in a loss in the user-fairness and the total system accuracy?
  %  \item \textbf{Q3}: Does the \underline{proposed CP-fairness} algorithm in this work meet the requirements for fairness on both the consumer and supplier sides simultaneously, and whether this comes at a cost in terms of overall system accuracy or not necessarily? 

\begin{table*}
\centering
\caption{Results for all models on \datasetB\ and \datasetE}
\label{tbl:results}
\small
\scalebox{0.75}{\begin{tabular}{llllllllllllllllll}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Type} & \multicolumn{7}{c}{Amazon Prime Pantry} && \multicolumn{7}{c}{Foursquare} \\
\cmidrule{3-9}\cmidrule{11-17}
                        &                       & Rec & NDCG & Cold & PF$_{eq}$ & PF$_{prop}$ & All $\uparrow$ & $\Delta$ $\uparrow$ && Rec & NDCG & Cold & PF$_{eq}$ & PF$_{prop}$ & All $\uparrow$ & $\Delta$ $\uparrow$ \\
\midrule
\multicolumn{17}{c}{\textbf{}} \\ \hline
%Random & - & 0.0035 & 0.0149 & 0.0029 & 0.6759 && 6.7339 & 0.77 & 0.1996 & 0.8004 & -0.6008 && 0.0807 & 23.05 & 0.0 \\
% MostPop & - & 0.0302 & 0.0566 & 0.0288 & 0.3258 && 3.7133 & 0.0049 & 1.0 & 0.0 & 1.0 && 0.7209 & 23.87 & 0.0 \\ \hline
BPR & A & 0.0043 & 0.0033 & 0.245 & 0.8894 & 0.0503 & 0.2662 & - && 0.0076 & 0.0063 & 0.2593 & 0.9588 & 0.0742 & 0.234 & - \\
BPR & c$^{0}$PF & 0.0151 & \cellcolor{purple!20}0.0085 & \cellcolor{purple!20}0.3384 & 1.0 & \cellcolor{purple!20}0.9842 & \cellcolor{purple!20}0.6005 & 1.2558 && 0.0508 & \cellcolor{purple!20}0.0249 & \cellcolor{purple!20}0.3144 & 1.0 & \cellcolor{purple!20}1.0 & \cellcolor{purple!20}0.5871 & 1.509 \\
BPR & c$^{0.2}$PF & 0.0138 & 0.0072 & 0.4713 & 1.0 & 0.9842 & 0.6024 & 1.263 && 0.0582 & 0.0279 & 0.3787 & 1.0 & 1.0 & 0.6313 & 1.6979 \\
%BPR & c$^{0.33}$PF & 0.0129 & 0.007 & 0.6209 & 1.0 & 0.9842 & 0.6458 & 1.426 && 0.0536 & 0.0268 & 0.4395 & 1.0 & 1.0 & 0.643 & 1.7479 \\
BPR & c$^{0.5}$PF & 0.0132 & 0.0057 & 0.8576 & 1.0 & 0.9842 & 0.6863 & 1.5781 && 0.0388 & 0.0222 & 0.5877 & 1.0 & 1.0 & 0.6576 & 1.8103 \\
BPR & c$^{1}$PF & 0.0129 & \cellcolor{purple!20}0.0058 & \cellcolor{purple!20}0.966 & 1.0 & \cellcolor{purple!20}0.9842 & \cellcolor{purple!20}\textbf{0.7241} & \textbf{1.7201} && 0.024 & 0.0107 & 0.9364 & 1.0 & 1.0 & 0.6858 & 1.9308 \\
%BPR & c$^{2}$PF & 0.0131 & 0.0056 & 0.9693 & 1.0 & 0.9842 & 0.7199 & 1.7044 && 0.0231 & 0.009 & 0.9752 & 1.0 & 1.0 & 0.686 & 1.9316 \\
BPR & c$^{5}$PF & 0.0131 & \cellcolor{purple!20}0.0056 & \cellcolor{purple!20}0.9693 & 1.0 & \cellcolor{purple!20}0.9842 & \cellcolor{purple!20}0.7199 & 1.7044 && 0.0231 & \cellcolor{purple!20}0.009 & \cellcolor{purple!20}0.9761 & 1.0 & 1.0 & \cellcolor{purple!20}\textbf{0.6863} & \textbf{1.9329} \\ \hline
NeuMF & A & 0.0057 & 0.004 & 0.2216 & 0.8292 & 0.0 & 0.4072 & - && 0.0085 & 0.0078 & 0.2488 & 0.9346 & 0.05 & 0.2969 & - \\
NeuMF & c$^{0}$PF & 0.0226 & \cellcolor{purple!20}0.0127 & \cellcolor{purple!20}0.3165 & 0.8877 & \cellcolor{purple!20}0.7535 & \cellcolor{purple!20}0.6441 & 0.5818 && 0.0582 & \cellcolor{purple!20}0.0299 & \cellcolor{purple!20}0.3131 & 1.0 & \cellcolor{purple!20}1.0 & \cellcolor{purple!20}0.6248 & 1.1044 \\
NeuMF & c$^{0.2}$PF & 0.02 & 0.011 & 0.4016 & 0.8877 & 0.7535 & 0.6217 & 0.5268 && 0.0545 & 0.0278 & 0.455 & 1.0 & 1.0 & 0.656 & 1.2095 \\
%NeuMF & c$^{0.33}$PF & 0.0174 & 0.0092 & 0.4321 & 0.8877 & 0.7535 & 0.5736 & 0.4086 && 0.0554 & 0.0256 & 0.4855 & 1.0 & 1.0 & 0.6495 & 1.1876 \\
NeuMF & c$^{0.5}$PF & 0.0181 & 0.0087 & 0.4711 & 0.8877 & 0.7535 & 0.5723 & 0.4055 && 0.0591 & 0.0281 & 0.5171 & 1.0 & 1.0 & 0.6789 & 1.2866 \\
NeuMF & c$^{1}$PF & 0.0192 & 0.0097 & 0.6017 & 0.8877 & 0.7535 & \textbf{0.646} & \textbf{0.5864} && 0.0452 & 0.0199 & 0.5944 & 1.0 & 1.0 & 0.642 & 1.1623 \\
%NeuMF & c$^{2}$PF & 0.014 & 0.0061 & 0.836 & 0.8877 & 0.7535 & 0.6139 & 0.5076 && 0.0332 & 0.0154 & 0.7128 & 1.0 & 1.0 & 0.6472 & 1.1799 \\
NeuMF & c$^{5}$PF & 0.0142 & \cellcolor{purple!20}0.0057 & \cellcolor{purple!20}0.9261 & 0.8877 & 0.7535 & \cellcolor{purple!20}0.6309 & 0.5494 && 0.036 & \cellcolor{purple!20}0.0145 & \cellcolor{purple!20}0.9453 & 1.0 & 1.0 & \cellcolor{purple!20}\textbf{0.7183} & \textbf{1.4193} \\ \hline
MultiVAE & A & 0.0047 & 0.0029 & 0.2149 & 0.8706 & 0.0324 & 0.1771 & - && 0.0128 & 0.0105 & 0.2239 & 0.8857 & 0.0 & 0.408 & - \\
MultiVAE & c$^{0}$PF & 0.0153 & \cellcolor{purple!20}0.008 & \cellcolor{purple!20}0.3188 & 0.9957 & \cellcolor{purple!20}0.9557 & \cellcolor{purple!20}0.566 & 2.1959 && 0.0729 & \cellcolor{purple!20}0.036 & \cellcolor{purple!20}0.2985 & 1.0 & \cellcolor{purple!20}0.9997 & \cellcolor{purple!20}0.6661 & 0.6326 \\
MultiVAE & c$^{0.2}$PF & 0.0155 & 0.0081 & 0.4845 & 0.9957 & 0.9557 & 0.6246 & 2.5268 && 0.0674 & 0.0343 & 0.4183 & 1.0 & 0.9999 & 0.6933 & 0.6993 \\
%MultiVAE & c$^{0.33}$PF & 0.0136 & 0.0059 & 0.7161 & 0.9957 & 0.9557 & 0.6361 & 2.5918 && 0.0536 & 0.0274 & 0.5878 & 1.0 & 0.9999 & 0.697 & 0.7083 \\
MultiVAE & c$^{0.5}$PF & 0.0146 & 0.0058 & 0.8964 & 0.9957 & 0.9557 & 0.6925 & 2.9102 && 0.0388 & \cellcolor{purple!20}0.0163 & 0.8436 & 1.0 & 0.9999 & 0.6976 & 0.7098 \\
MultiVAE & c$^{1}$PF & 0.0142 & \cellcolor{purple!20}0.0055 & \cellcolor{purple!20}0.9421 & 0.9957 & \cellcolor{purple!20}0.9557 & \cellcolor{purple!20}0.698 & 2.9413 && 0.0342 & 0.0137 & \cellcolor{purple!20}0.9656 & 1.0 & \cellcolor{purple!20}0.9999 & \cellcolor{purple!20}\textbf{0.7189} & \textbf{0.762} \\
%MultiVAE & c$^{2}$PF & 0.0144 & 0.0057 & 0.9435 & 0.9957 & 0.9557 & \textbf{0.7044} & \textbf{2.9774} && 0.0332 & 0.0132 & 0.9691 & 1.0 & 0.9999 & 0.7162 & 0.7554 \\
MultiVAE & c$^{5}$PF & 0.0144 & \cellcolor{purple!20}0.0057 & \cellcolor{purple!20}0.9435 & 0.9957 & \cellcolor{purple!20}0.9557 & \cellcolor{purple!20}\textbf{0.7044} & \textbf{2.9774} && 0.0323 & 0.0129 & \cellcolor{purple!20}0.9691 & 1.0 & \cellcolor{purple!20}0.9999 & \cellcolor{purple!20}0.7138 & 0.7495 \\ \hline
LightGCN & A & 0.0051 & 0.0033 & 0.2408 & 1.0 & 0.1891 & 0.3085 & - && 0.008 & 0.0069 & 0.2511 & 0.9816 & 0.1013 & 0.2705 & - \\
LightGCN & c$^{0}$PF & 0.0183 & \cellcolor{purple!20}0.0089 & \cellcolor{purple!20}0.3271 & 0.9785 & \cellcolor{purple!20}0.9182 & 0.5857 & 0.8985 && 0.0563 & \cellcolor{purple!20}0.0275 & \cellcolor{purple!20}0.3066 & 0.9996 & \cellcolor{purple!20}0.987 & \cellcolor{purple!20}0.5998 & 1.2174 \\
LightGCN & c$^{0.2}$PF & 0.0149 & 0.0069 & 0.4649 & 0.9785 & 0.9182 & 0.5701 & 0.848 && 0.0526 & 0.0276 & 0.3867 & 1.0 & 0.9999 & 0.632 & 1.3364 \\
%LightGCN & c$^{0.33}$PF & 0.0177 & 0.008 & 0.661 & 0.9785 & 0.9182 & 0.6702 & 1.1724 && 0.0434 & 0.0225 & 0.4964 & 1.0 & 0.9999 & 0.6295 & 1.3272 \\
LightGCN & c$^{0.5}$PF & 0.0147 & 0.0061 & 0.8167 & 0.9785 & 0.9182 & 0.6613 & 1.1436 && 0.0379 & 0.0168 & 0.722 & 1.0 & 0.9999 & 0.6608 & 1.4429 \\
LightGCN & c$^{1}$PF & 0.0129 & \cellcolor{purple!20}0.0052 & \cellcolor{purple!20}0.9345 & 0.9785 & 0.9182 & \cellcolor{purple!20}0.6741 & 1.1851 && 0.0277 & \cellcolor{purple!20}0.0103 & \cellcolor{purple!20}0.9437 & 1.0 & \cellcolor{purple!20}0.9999 & \cellcolor{purple!20}0.6855 & 1.5342 \\
%LightGCN & c$^{2}$PF & 0.0129 & 0.0051 & 0.955 & 0.9785 & 0.9182 & \textbf{0.6766} & \textbf{1.1932} && 0.0277 & \cellcolor{purple!20}0.0105 & \cellcolor{purple!20}0.9739 & 1.0 & \cellcolor{purple!20}0.9999 & \cellcolor{purple!20}0.6968 & 1.576 \\
LightGCN & c$^{5}$PF & 0.0127 & 0.005 & \cellcolor{purple!20}0.9559 & 0.9785 & 0.9182 & \cellcolor{purple!20}0.6736 & 1.1835 && 0.0277 & 0.0105 & 0.9748 & 1.0 & 0.9999 & \textbf{0.6976} & \textbf{1.5789} \\ \hline
NGCF & A & 0.0032 & 0.0025 & 0.241 & 0.9208 & 0.0861 & 0.109 & - && 0.0046 & 0.0039 & 0.2475 & 1.0 & 0.1544 & 0.134 & - \\
NGCF & c$^{0}$PF & 0.014 & \cellcolor{purple!20}0.0076 & \cellcolor{purple!20}0.3328 & \cellcolor{purple!20}0.9941 & \cellcolor{purple!20}0.9647 & \cellcolor{purple!20}0.5641 & 4.1752 && 0.0314 & \cellcolor{purple!20}0.0174 & \cellcolor{purple!20}0.3057 & 0.9861 & \cellcolor{purple!20}0.9555 & \cellcolor{purple!20}0.5117 & 2.8187 \\
NGCF & c$^{0.2}$PF & 0.0129 & 0.0064 & 0.4762 & 0.9941 & 0.9647 & 0.5749 & 4.2743 && 0.0323 & 0.0172 & 0.4492 & 0.9861 & 0.9555 & 0.5586 & 3.1687 \\
%NGCF & c$^{0.33}$PF & 0.0155 & 0.0074 & 0.6368 & 0.9941 & 0.9647 & 0.6574 & 5.0312 && 0.0351 & \cellcolor{purple!20}0.0206 & \cellcolor{purple!20}0.6144 & 0.9861 & 0.9555 & \cellcolor{purple!20}0.6396 & 3.7731 \\
NGCF & c$^{0.5}$PF & 0.0159 & 0.0069 & 0.8648 & 0.9941 & 0.9647 & \cellcolor{purple!20}\textbf{0.719} & \textbf{5.5963} && 0.024 & 0.0107 & 0.8127 & 0.9861 & 0.9555 & 0.6298 & 3.7 \\
NGCF & c$^{1}$PF & 0.014 & 0.0052 & 0.9618 & 0.9941 & 0.9647 & 0.6985 & 5.4083 && 0.0259 & 0.0103 & \cellcolor{purple!20}0.9455 & 0.9861 & 0.9555 & \cellcolor{purple!20}0.6708 & 4.006 \\
%NGCF & c$^{2}$PF & 0.0138 & 0.0051 & \cellcolor{purple!20}0.9644 & 0.9941 & \cellcolor{purple!20}0.9647 & \cellcolor{purple!20}0.6968 & 5.3927 && 0.0259 & 0.01 & \cellcolor{purple!20}0.9599 & 0.9861 & 0.9555 & \cellcolor{white!20}0.6741 & 4.0306 \\
NGCF & c$^{5}$PF & 0.0138 & 0.0051 & 0.9644 & 0.9941 & 0.9647 & 0.6968 & 5.3927 && 0.0259 & 0.01 & 0.9604 & 0.9861 & 0.9555 & \textbf{0.6742} & \textbf{4.0313} \\
\bottomrule
\end{tabular}}
\end{table*}

\begin{table*}
\centering
\caption{Aggregated results for all datasets.}
\small
\begin{tabular}{lllllllllllllll}
\toprule
\multirow{2}{*}{Type} & \multicolumn{2}{c}{MovieLens100K} && \multicolumn{2}{c}{Prime Pantry} && \multicolumn{2}{c}{Luxury Beauty} && \multicolumn{2}{c}{LastFM} && \multicolumn{2}{c}{Foursquare} \\
\cmidrule{2-3}\cmidrule{5-6}\cmidrule{8-9}\cmidrule{11-12}\cmidrule{14-15}
                        &                        All $\uparrow$ & $\Delta$ $\uparrow$ && All $\uparrow$ & $\Delta$ $\uparrow$ && All $\uparrow$ & $\Delta$ $\uparrow$ && All $\uparrow$ & $\Delta$ $\uparrow$ && All $\uparrow$ & $\Delta$ $\uparrow$ \\
\midrule
\multicolumn{15}{c}{\textbf{}} \\ \hline
A & 0.242 & - && 0.254 & - && 0.258 & - && 0.206 & - && 0.269 & - \\
c$^{0.5}$PF & 0.546 & 2.286 && 0.666 & 2.327 && 0.65 & 1.821 && 0.617 & 2.665 && 0.665 & 1.79 \\
c$^{1}$PF & \textbf{0.548} & \textbf{2.302} && \textbf{0.688} & \textbf{2.368} && 0.677 & 1.993 && 0.639 & 2.818 && 0.681 & 1.879 \\
c$^{5}$PF & 0.548 & 2.252 && 0.685 & 2.353 && 0.737 & 2.323 && \textbf{0.642} & \textbf{2.907} && \textbf{0.698} & \textbf{1.96} \\
\bottomrule
\end{tabular}
\end{table*}

\noindent \textbf{Discussion.} We begin our experimental study by
addressing the above evaluation questions. We report the detailed
performance results of two datasets, \datasetB\ and \datasetE\ (out of the 5 we employ and described) in Table 3, due to space constraints. However, using the boxplots provided in Figure xxxx, we are able to represent the aggregate average findings across all of the datasets in a graphical format. Note that the metric $nPF$has been used to combine the three evaluation objectives (accuracy, novelty and $PF_{prop}$), which be do using the eighted 

\vspace{0.75em} \noindent \textbf{RQ1: Fairness-Enhancement Performance}

\begin{itemize}
    \item \textbf{Overall trend.} For this purpose, we consider the values obtained by All (combined accuracy, coldness and fairness metric) and the associated enhancements $\Delta$. In general, one can note that one of the variants of c$^{\gamma}$PF enhances the system's performance on each particular metric and as a whole. For the \datasetB\ dataset, for the models \texttt{BPR}, \texttt{MultiVAE} and \texttt{NGCF}, we have the best All values being 0.7241, 0.7044, 0.719 and the corresponding delta values being 1.7201, 2.9774, 5.5963. It is important to note how the highest $\gamma$ values tend to lead to the best performance (c$^{1}$PF, c$^{2}$PF, c$^{5}$PF). The results are consistent across both datasets.
    \item \textbf{Per-model analysis.} Among the models we employ, NGCF shows the best performance in terms of $\Delta$, i.e. enhancement, on both datasets, with all the values in the range 2-6, and the best ones being 5.5963 and 4.0313, respectively.
    \item \textbf{Consistency across datasets.} As said above, both datasets show a similar trend. However, it turns out that the amount of dataset characteristics can impact the improvement: for example, on \datasetB,\ \texttt{MultiVAE} achieves a $\Delta$ performance of 2.9774 while on \datasetE, it is only 0.762.
\end{itemize}

\vspace{0.75em} \noindent \textbf{RQ2: Parameters Impact and Calibration}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{source}
    \caption{NDCG, Novelty, MAD and All combined for the different combinations of $\gamma$ and $\lambda$ using BPR}
\end{figure*}

\begin{itemize}
    \item \textbf{Per-parameter considerations.} Say how differently parameters impact the 4 considered dimensions, and maybe also other data we remember/know and comment on their weight in the All heatmap.
    \item \textbf{Metrics trade-off.} Spot trade-off in the heatmaps and state doable trade-off from the conducted experiments. 
\end{itemize}
